Client-supervised Federated Learning: Towards One-model-for-all Personalization

Personalized Federated Learning (PerFL) is a new machine learning paradigm that delivers personalized models for diverse clients under federated learning settings. Most PerFL methods require extra learning processes on a client to adapt a globally shared model to the client-specific personalized model using its own local data. However, the model adaptation process in PerFL is still an open challenge in the stage of model deployment and test time. This work tackles the challenge by proposing a novel federated learning framework to learn only one robust global model to achieve competitive performance to those personalized models on unseen/test clients in the FL system. Specifically, we design a new Client-Supervised Federated Learning (FedCS) to unravel clients' bias on instances' latent representations so that the global model can learn both client-specific and client-agnostic knowledge. Experimental study shows that the FedCS can learn a robust FL global model for the changing data distributions of unseen/test clients. The FedCS's global model can be directly deployed to the test clients while achieving comparable performance to other personalized FL methods that require model adaptation.

==> gmqsdyrtmmygsjqmkqwdsmzsbpgdwbhv/icme24_1_introduction.tex <==
Modern machine learning relies on massive data to train models like deep neural networks (DNNs), but collecting data is becoming more sensitive with increasing attention to privacy protection. Then, federated learning (FL)~\cite{mcmahan2017communication} emerged and became a popular learning paradigm in recent years. The FL aims to coordinate a set of clients (i.e., devices) to train a global model while preserving their data locally and privately. Further, personalized FL (PerFL)~\cite{deng2020adaptive,mansour2020three,wu2022motley} balances cross-client training and personalization. Clients will collaborate as in vanilla FL and leverage client-specific properties to learn personalized models demonstrating superior performance on non-IID data.

Existing personalized federated learning research usually aims to learn many client-specific personalized models to tackle the non-IID data in federated learning systems. Specifically, a global model will be learned to grasp shared knowledge, and then many personalized models will be learned or fine-tuned on the client by leveraging the global model and local dataset. Although this client-specific personalised model strategy has the potential to catch non-IID in fine-grained, the on-device learning and fine-tuning process is usually difficult to control in practice, especially in the stage of model deployment and test time.

This paper aims to rethink the personalized federated learning problem by proposing a one-model-for-all strategy to embody personalization in federated settings. One motivation is that model personalization in most PerFL methods relies on the bias of instances on the same client, and little supervised information describing the client is introduced. Then, the global model trained on the same data will attain the same performance if it can recognize the bias of a client. Inspired by this, we propose to use a one-model-for-all strategy to learn a unified model that can be shared across clients in the FL system. Moreover, the client-specific information will be encoded in a unified representation space and then be fed into a decision module along with the client-agnostic knowledge to make the final prediction.

Based on the thought above, this work proposes a novel \textbf{Client-Supervised Federated Learning (FedCS)} that is to learn a unified global model with the below functions, including 1) to learn a unified representation space that can encode the bias of a client, 2) to share client-agnostic knowledge as vanilla FL methods, and 3) to make personalized predictions by leveraging both pieces of information. Moreover, the \textbf{Representation Alignment (RA)} mechanism in FedCS could become a plug-in component to be integrated with any federated learning methods. It enables a vanilla FL model to output personalized results without on-device fine-tuning steps. An illustration of the FedCS is in~Fig.\ref{fig:architecture}.

% Specifically, the neural architecture of the new FL framework will be composed of three modules that are the backbone for representation learning, an extra projection layer for client decorrelation, and fully-connected layers for decisions or predictions. 


\begin{figure}[t]
%\begin{minipage}[b]{1.0\linewidth}
  \centerline{\epsfig{figure=images/Fig-Architecture.png,width=8.5cm}}
  % \vspace{1.5cm}
  % \centerline{(a) Result 1}\medskips
%\end{minipage}
% \hfill
% \begin{minipage}
% \end{minipage}
%
\caption{Illustration to the FedCS. (b) and (c) describe distributions of instances' latent representations before and after the Representation Alignment module (RA Module). Types of markers denote classes, and colors indicate clients they are observed. The vanilla feature extractor is unable to recognize clients' bias. RA module in FedCS will align the hidden space so that latent representations can indicate biases of clients.}
\label{fig:architecture}
\end{figure}


% The projection layer of client decorrelation is to decompose the instance's representation into two separated spaces: a client-specific representation space, and a universal representation space. It imposes orthogonality constraints on each space, restricting their outputs to vary along with axes aligned with client-specific or client-agnostic knowledge. An instance will then have two uncorrelated representations based on spans of axes regarding different types of knowledge. We call them \textbf{CRep} (i.e., \textbf{\textit{client-specific representation}}) and \textbf{URep} (i.e., \textbf{\textit{universal representation}}).

To learn the above objectives in a federated optimization framework, we designed a novel \textbf{Client-Supervised Federated Optimization Framework} to align the objective representation space while being consistent with the federated optimization framework. It exploits the bias that instances on the same client are influenced by identical client properties and formulates the representation aligning task into an optimization problem that clients can solve collaboratively. % Then it infers axes of client-agnostic knowledge through the Gram-Schmidt process~\cite{strang2021introduction}, which guarantees that the CRep and URep are complementary in representing instances.

Through qualitative and quantitative experiments, we illustrate how FedCS is integrated into a black-box model to achieve compared performance of other personalized federated learning methods. %We verify CRep's consistency with client properties contributing to personalization and illuminate how they cooperate with FL models to induce personalized outputs.
Moreover, we demonstrate that FedCS is compatible with most FL models. Vanilla models with an RA module can achieve competitive performance compared to those ad hoc PerFL models while not need extra fine-tuning steps or personal parameters.

The main contributions are summarized as follows:
\begin{itemize}
\item We propose a novel one-model-for-all personalized FL framework that won't require an extra fine-tuning process at the stage of model deployment and test time. The personalization in the FL system is carried on representations indicating client bias rather than models.

\item We designed a novel \textbf{representation alignment} mechanism to project instances' representation into a space indicating clients' biases. The following decision layers in the neural architecture can automatically learn to make personalized predictions by leveraging the client's bias.

\item A \textbf{client-supervised optimization framework} is designed to fit the proposed framework. It formulates the representation-aligning problem into a unified optimization framework that clients can solve collaboratively under FL settings.

\item Contrast with baseline methods shows that, by integrating FedCS into vanilla FL models, they can achieve competitive personalization performance without requiring extra fine-tuning steps or personal parameters.
\end{itemize}

==> gmqsdyrtmmygsjqmkqwdsmzsbpgdwbhv/icme24_2_related_work.tex <==
% \subsection{Personalized Federated Learning}
\textbf{Federated Learning} is an emerging machine learning paradigm where many clients collaborate to train a global model by sharing and aggregating model parameters rather than user data~\cite{mcmahan2017communication}. %,reddi2020adaptive \cite{mcmahan2017communication} proposed a fundamental framework, FedAvg, where 
Further work~\cite{deng2020adaptive,mansour2020three,wu2022motley} shows that the global model performs better after tuning toward client-specific properties and proposes \textbf{Personalized Federated Learning}.

% \subsubsection{Fully Personalization} //TODO
A popular way to personalize is to fine-tune the global model on a client's local data~\cite{mcmahan2017communication,cheng2021fine,collins2022fedavg}; meta-learning strategies will help improve the tuning process~\cite{jiang2019improving,fallah2020personalized}. Meanwhile, \cite{li2021ditto} trains a local model for each client while constraining the distributed training procedures with a shared regularizer. %\cite{shamsian2021personalized} proposes to learn a hyper-network that will generate personalized parameters according to clients' local data. However, by these methods, client-specific and client-agnostic knowledge will be entangled and scattered throughout the entire model so that the whole global model has to be tuned on local data to be adapted to its bias.
% \subsubsection{Partially Personalization} //TODO
Recent work~\cite{pillutla2022federated} studies partial personalization, splitting an FL model into global and local parts. Personalization is fulfilled by individually training the local part of a model on clients. \cite{li2021fedbn} is a simple but efficient case of these methods. It trains a model through the vanilla FedAvg~\cite{mcmahan2017communication} except for preserving batch-normalization modules locally.~\cite{collins2021exploiting} introduces a method to learn a shared data representation across clients and unique classification heads for each client. \cite{luo2022disentangled} utilizes a global and a local encoder to learn different representations for cross-client collaboration and personalization. \cite{ye2023upfl} and \cite{sun2022feature} propose to learn unique representations for client properties to improve personalization on new clients. However, these methods require extra training data to capture those clients' properties when deployed on them, which is only sometimes feasible.

% \subsubsection{Group-wise Personalization} //TODO
% Unsupervised methods~\cite{ghosh2020efficient, mansour2020three} indicate that clients could be clustered into groups regarding their properties. Then the model shared within a group will perform similarly to those locally fine-tuned ones. \cite{wu2022motley} validates that the cluster structure of these models is consistent with the natural cluster structure of client properties, e.g., clusters of English and Spanish users. \cite{zhu2021diurnal} shows that underlying daytime and nighttime modes involve clients' properties. It formulates this prior into latent variables and clusters clients to improve personalization performance by the Expectation-Maximum. Unfortunately, clustering is sensitive to multiple factors, e.g., the number of clusters. It is hard to select hyper-parameters to ensure the resulting cluster structure can be properly interpreted~\cite{wu2022motley}. Besides, restricted by FL's privacy policy, existing methods rely on model parameters to measure client similarity. \cite{ghosh2020efficient,wu2022motley} demonstrate that this strategy could be unreliable in practice for problems like mode collapse and high communication costs.

%\subsection{Interpretable Machine Learning}
%\label{Interpretable Machine Learning}
%\textbf{Interpretable Machine Learning} is a field studying the comprehensibility of machine learning models. It aims to illustrate why specific predictions are made by a model~\cite{kim2016examples,miller2019explanation} and reveals knowledge either contained in data or learned by the model~\cite{murdoch2019definitions}. Traditional statistical models like linear regression and decision trees are essentially interpretable, but they have limited capacity to handle complex problems like image recognition. So recent research focuses on disclosing knowledge in deep models that are more powerful and complicated.

%The most extensively discussed interpreting method is visualizing feature attributions by propagating gradients~\cite{simonyan2013deep,selvaraju2017grad} or calculating the Shapley value~\cite{lundberg2017unified,sundararajan2017axiomatic}. However, although various works attempt to verify the interpretability of existing attribution maps~\cite{chattopadhay2018grad, draelos2020use,sundararajan2020many}, there is still controversy if their interpretation was consistent with the ground truth knowledge~\cite{adebayo2018sanity,kindermans2019reliability,tomsett2020sanity}.

%\textbf{Concept Vectors and Concept Whitening} are new ways to investigate the decision process of a black-box model~\cite{kim2018interpretability,ghorbani2019towards,koh2020concept,chen2020concept}. These approaches learn a set of concept vectors, i.e., decision hyperplanes aligned with certain concepts, to classify hidden units inside a DNN. End users can unravel concepts leading to a specific output by inspecting whether relevant hidden units are activated. Notably, the concept vector method allows human-in-the-loop operations to test and quantify a concept's influence, which is critical in studying the causation of a prediction~\cite{kim2018interpretability,koh2020concept}. A disadvantage is that these methods require supervised information for each concept, either by auxiliary datasets~\cite{kim2018interpretability,chen2020concept} or labels~\cite{ghorbani2019towards,koh2020concept}. Then they are limited to work in scenarios where concepts of interest are enumerable and easily depicted, but this is only the case for some applications.

==> gmqsdyrtmmygsjqmkqwdsmzsbpgdwbhv/icme24_3_problem_formulation.tex <==
\textbf{Federated Learning (FL)} assumes $K$ clients participate in a learning process with ${\{}\mathbf{x}_1^{(i)}, \mathbf{x}_2^{(i)},...,\mathbf{x}_{N_i}^{(i)} \}\in \mathcal{X}^{(i)}$ denoting instances on the $i$-th client, and $\{y_1^{(i)},y_2^{(i)},...,y_{N_i}^{(i)}\}\in \mathcal{Y}^{(i)}$ are their labels. The FL task is to find the optimal parameters $\omega^{*}$ for a global model $f(\mathbf{x};\omega)$ by minimising the total loss of all clients as the following optimization problem:

% \begin{eqnarray}
% y &=& ax^2+bx+c \nonumber \\
% ~ &=& (x+p)(x+q)
% \end{eqnarray}
% shows an example of an equation layout.

\begin{equation}
    \label{def-fl}
    \begin{aligned}
    \omega^{*}=\arg\min_{\omega}\sum_{i=1}^{K}\alpha_i \mathcal{L}_i(\omega)
    \end{aligned}
\end{equation}

where $\mathcal{L}_i(\omega)=(1/N_i)\sum_{j=1}^{N_i}l(f(\mathbf{x}_j^{(i)};\omega),y_{j}^{(i)})$ is the supervised loss on the $i$-th client, and $\alpha_i$ is its weight. In particular, in the standard FL framework~\cite{mcmahan2017communication}, $\alpha_i$ is the fraction of the size of the client's training data, i.e., $\alpha_i= N_i/\sum_{i'=1}^{K}N_{i'}$. Each client will update $\omega$ privately by minimizing $\mathcal{L}_i(\omega)$, and a server will orchestrate the distributed training process by collecting locally updated $\omega$ and synchronizing the averaged one.

\textbf{Personalized Federated Learning (PerFL)} leverages cross-client collaboration but learns a personalized model $f(\mathbf{x};\omega,\mu_i)$ for each client, where $\omega$ denotes parameters shared, and $\mu_i$ denotes parameters for the $i$-th client. The learning task can be formulated into a unified optimization problem~\cite{pillutla2022federated}:
\begin{equation}
    \label{def-perfl}
    \begin{aligned}
    \omega^{*},\{\mu_i^{*}\}_{i=1}^{K}=\arg\min_{\omega,\{\mu_i\}_{i=1}^{K}}\sum_{i=1}^{K}\alpha_i\mathcal{L}_i(\omega, \mu_i)
    \end{aligned}
\end{equation}
There are different types of personalization according to how to define $\omega$ and $\mu_i$. 1) \textbf{full personalization}: a local model is fully parameterized by $\mu_i$, and the global model guides the local training process, e.g., regularizing $\mu_i$ by minimizing $\|\omega-\mu_i\|_2$~\cite{li2021ditto} or initializing local parameters with $\mu_i= \omega-\nabla\mathcal{L}_i$~\cite{fallah2020personalized}; 2) \textbf{partial personalization}: $\omega$ and $\mu_i$ constitute the global and personal parts of a local model, where $\omega$ is shared through the fundamental FL method in \ref{def-fl}, and $\mu_i$ is trained individually on each client. e.g., $\omega$ could be parameters of a shared backbone model, and $\mu_i$ is a classification head for the $i$-th client~\cite{collins2021exploiting}. %and 3) \textbf{group-wise personalization}: clients are clustered into groups to maintain a personalized model within each group, e.g., for clients in the group $G_c$, there is $\omega_c= \sum \alpha_i \mu_i[i\in G_c]$~\cite{ghosh2020efficient,mansour2020three}.

==> gmqsdyrtmmygsjqmkqwdsmzsbpgdwbhv/icme24_4_methodology.tex <==
Looking inside the latent space of a DNN $f(\mathbf{x};\omega)=g(h(\mathbf{x};\omega_h);\omega_g)$, it consists of two parts: $h(\mathbf{x};\omega_h)$ is a feature extractor learning the latent representation $\mathbf{z}\in\mathbb{R}^{d}$, and $g(\mathbf{z};\omega_g)$ is a classification head making predictions based on $\mathbf{z}$. Our goal is to align the latent representation space for $\mathbf{z}$, such that 1) it is able to embed client-specific information, i.e., instances from similar clients will have similar values and vary significantly otherwise; 2) it is able to share client-agnostic knowledge as vanilla FL methods, and 3) downstream modules can make personalized predictions by leveraging both information.

% personalization is transparent and interpretable. Specifically, $\mathbf{z}_p$ will vary along with changes in clients' properties, and one can inspect its influences on an FL model's personalized outputs.

% \subsection{Client Decorrelation}
Formally, FedCS looks for a projection $\mathbf{c}=\mathbf{P}^{T}\mathbf{z}$, where $\mathbf{P}_{d\times r}=[\mathbf{p}_1,\mathbf{p}_2,...,\mathbf{p}_r]$ is the orthonormal basis of the objective representation space. It searches for the optimal directions $\mathbf{P}^{*}$ according to an inductive bias that representation $\mathbf{c}$ on the same client shall be similar, and those from different clients are on the contrary.

\subsection{Representation Alignment}
Specifically, let $\bar{\mathbf{c}}^{(i)}$ denote the mean of representations on the $i$-th client, and $\bar{\mathbf{c}}$ be the global mean among clients.
\begin{equation}
    \begin{aligned}
    \Sigma_W=\frac{1}{\sum_{i=1}^{K}N_{i}}\sum_{i=1}^{K}\sum_{j=1}^{N_i}(\mathbf{c}_j^{(i)}-\bar{\mathbf{c}}^{(i)})(\mathbf{c}_j^{(i)}-\bar{\mathbf{c}}^{(i)})^{T}
    \end{aligned}
    \label{def-within-client-scatter-matrix}
\end{equation}
Eq.\ref{def-within-client-scatter-matrix} is the within-client scatter matrix that measures the scatter of latent representations within each client and
\begin{equation}
    \begin{aligned}
    \Sigma_B=\frac{1}{\sum_{i=1}^{K}N_{i}}\sum_{i=1}^{K}N_i(\bar{\mathbf{c}}^{(i)}-\bar{\mathbf{c}})(\bar{\mathbf{c}}^{(i)}-\bar{\mathbf{c}})^{T}
    \end{aligned}
    \label{def-between-client-scatter-matrix}
\end{equation}
Eq.\ref{def-between-client-scatter-matrix} is the between-client scatter matrix that measures the scatters of the mean across clients. To find the $\mathbf{P}^{*}$ is to find the directions that minimize $\Sigma_W$ and maximize $\Sigma_B$. For example, it can be formulated as the Linear Discriminate Analysis (LDA) problem below
\begin{equation}
    \mathbf{P}^{*}=\arg\max_{\mathbf{P}}J(\mathbf{P})=\arg\max_{\mathbf{P}}\text{Tr}(\Sigma_W^{-1}\Sigma_B)
    \label{def-rayleigh-quotient}
\end{equation}
where $\text{Tr}(\cdot)$ denotes the trace of the matrix.

Then, bring Eq.\ref{def-rayleigh-quotient} into the FL framework, the overall learning task is formulated as a bi-level optimization problem
%Particularly, as the original representation space in the DNN contains both client-specific/-irrelevant knowledge to make the decision, 
%to ensure that $\mathbf{P}$ and $\mathbf{Q}$ are complementary to contain the information in the original representation space, 
% Meanwhile, it worth noting that, for any instance, its CRep $\mathbf{c}$ and URep $\mathbf{s}$ are uncorrelated but not independent (appendix xxx). Decorrelate CRep influences from $\mathbf{z}$, we get the URep. It is implemented by the $\textbf{Gram-Schmidt process}$ (appendix xxx). Then the loss of xx is xxxxx.
\begin{equation}
    \begin{aligned}
    \omega_h^{*},\omega_g^{*} ~&=\arg\min_{\omega_h,\omega_g}\sum_{i=1}^{K}\alpha_i\mathcal{L}_i(\omega_h,\omega_g)\\
    s.t.~&\mathbf{P}^{*}=\arg\max_{\mathbf{P}}J(\mathbf{P})\\
    % ~&\mathbf{Q}^{*}=GSP(\mathbf{P}^{*})
    % s.t.~&\mathbf{P}^{*}=\arg\min_{\mathbf{P}}\text{Tr}(\sum_{i=1}^{K}\mathbf{M}_{W}\mathbf{M}_G^{-1})\\
    % &[\mathbf{P};\mathbf{Q}]^T[\mathbf{P};\mathbf{Q}] = \mathbf{I}_d
    \label{def-overall-loss}
    \end{aligned}
\end{equation}
where 
\begin{equation}
    \begin{aligned}
    \mathcal{L}_i=\sum_{j=1}^{N_{i}}l(g(\mathbf{P}^{T}h(\mathbf{x}_j^{(i)};\omega_h);\omega_g),y_j^{(i)})\\
    \label{def-overall-loss-local}
    \end{aligned}
\end{equation}
In the next section, we introduce a client-supervised method to optimize the Eq.\ref{def-overall-loss} under the FL setting.

\subsection{Client Supervised Optimization}
Theoretically, the optima of Eq.\ref{def-rayleigh-quotient} are eigenvectors of $\Sigma_{W}^{-1}\Sigma_{B}$ associated with the $r$ largest eigenvalues~\cite{duda2006pattern}. Then, the classification and the alignment tasks in Eq.\ref{def-overall-loss} can be optimized alternatively under the conventional FL framework~\cite{li2021ditto, pillutla2022federated}. However, decomposing $\Sigma_{W}^{-1}\Sigma_{B}$ is computationally expensive, and involves collecting the local mean $\bar{\mathbf{c}}^{(i)}$ which is privacy sensitive. To this end, we propose a client-supervised method that decomposes the learning task in Eq.\ref{def-rayleigh-quotient} into sub-tasks so that clients can optimize it collaboratively. % Differential privacy is applied to protect private information.

Concretely, previous works~\cite{ghassabeh2015fast} show that maximizing Eq.\ref{def-rayleigh-quotient} is equivalent to maximizing $\Sigma_W^{-1/2}\Phi\Sigma_W^{-1/2}$, where $\Phi$ is an approximation to the eigen system of the global correlation matrix $\Sigma_W+\Sigma_B$, and both $\Sigma_W^{-1/2}$ and $\Phi$ can be updated incrementally through the following equations
\begin{equation}
\begin{aligned}
    \Sigma_W^{-1/2} = \Sigma_W^{-1/2} + \eta * (I - \Sigma_W^{-1/2}\Sigma_W\Sigma_W^{-1/2})
    \label{eq-sigma}
\end{aligned}
\end{equation}
and 
\begin{equation}
\begin{aligned}
    \Phi = \Phi + \lambda * (\mathbf{\bar{u}}\mathbf{\bar{u}}^{T}\Phi - \Phi\tau(\Phi\mathbf{\bar{u}}\mathbf{\bar{u}}^{T}\Phi)
    \label{eq-phi}
\end{aligned}
\end{equation}
where $\mathbf{u} = \Sigma_W^{-1/2} \mathbf{\bar{c}}$, and $\tau(\cdot)$ is an operator that sets all the elements below the main diagonal of the matrix to zero. In this process, $\Sigma_W$ summarizes the correlation of instances on each client and hence will work as supervised information to encode the bias of a client into $\mathbf{u}$. Details of the derivations of Eq.\ref{eq-sigma} and Eq.\ref{eq-phi} are discussed in Appendix. Then, the representation alignment process is described in Algorithm.\ref{alg:representation alginment}, and the overall FL process with FedCS is described in Algorithm.\ref{alg:client supervised optimization}.
\begin{algorithm}[tb]
   \caption{Representation Alignment}
   \label{alg:representation alginment}
\begin{algorithmic}
   \STATE {\bfseries Input:} a batch of latent representations $\mathbf{z}$, global mean $\mathbf{z}_{g}$, client's local correlation $\Sigma_W^{-1/2}$ and $\Phi$
   \STATE {\bfseries begin:}
   \STATE 1. if $\Sigma_W^{-1/2}$ and $\Phi$ are empty, initialize $\Sigma_W^{-1/2}$ and $\Phi$
   \STATE 2. calculate local mean: $\mathbf{z}_{l} = mean(\mathbf{z})$
   \STATE 3. update global mean: $\mathbf{z}_{g} = \mathbf{z}_{g} + \frac{1}{|\mathbf{z}|}(\mathbf{z}-\mathbf{z}_{g})$
   \STATE 4. calculate local correlations: $\Sigma_{W}=(\mathbf{z}-\mathbf{z}_{l})(\mathbf{z}-\mathbf{z}_{l})^{T}$
   \STATE 5. update $\Sigma_W^{-1/2}$ by Eq.\ref{eq-sigma}
   \STATE 6. update $\Phi$ by Eq.\ref{eq-phi}
   \STATE 7. $\mathbf{P}=\Sigma_W^{-1/2}\Phi$
   \STATE 8. return $\mathbf{P}$
   \STATE{\bfseries end}
\end{algorithmic}
\end{algorithm}

% \begin{equation}
%     1. update local correelation mtx
%     2. inv_sqrt_local_correlation = inv_sqrt_local_correlation + lr * (I - inv_sqrt_local_correlation client_cor inv_sqrt_local_correlation)
%     3. u = inv_sqrt_local_correlation * global_mean
%     4. u_cor = u@u^t
%     5. phi = phi + lr * (u_cor * phi - phi * triu(phi *u_cor * phi)
%     6. P = inv_sqrt * phi
% \end{equation}


\begin{algorithm}[tb]
   \caption{Client-Supervised Federate Learning}
   \label{alg:client supervised optimization}
\begin{algorithmic}
   \STATE {\bfseries Input:} training data $(\mathcal{X}^{(i)},\mathcal{Y}^{(i)})$ distributed on $K$ clients, $t$ the round to update $P$.
   \STATE {\bfseries begin:}
   \STATE 1. Initialize the FL model $f(\mathbf{x};\omega)=g(h(\mathbf{x};\omega_h);\omega_g)$.
   \STATE 2. Select a set of clients $\mathbb{S}$
   \STATE {\bfseries for} the $i$-th client in $\mathbb{S}$ {\bfseries parallel do}
   \STATE ~ update $\omega_h$ and $\omega_g$ locally
   \STATE ~ if round\%$t$ == 0:
   \STATE ~ update $\mathbf{P}$ locally by Algorithm.\ref{alg:client supervised optimization}
   \STATE {\bfseries end for}
   \STATE 3. Aggregate local updates of $\omega_h$, $\omega_g$ and $\mathbf{P}$ by averaging
   \STATE{\bfseries end}
\end{algorithmic}
\end{algorithm}

==> gmqsdyrtmmygsjqmkqwdsmzsbpgdwbhv/icme24_5_experiments.tex <==
In this section, we demonstrate the advantages of FedCS in learning from clients with non-i.i.d. data. The FedCS can learn a robust FL global model for the changing data distributions of unseen/test clients. The FedCS's global model can be directly deployed to the test clients while achieving comparable performance to other personalized FL methods that require model adaptation.

\subsection{Client Settings}
We simulate FL environments by allocating instances from benchmark datasets to 50 clients, and two types of heterogeneity are applied (Details of client settings are introduced in the Appendix).
\begin{itemize}
\item \textbf{Label-shift}: We experiment, respectively, on the MNIST and the CIFAR-10 datasets. We allocate instances of each label individually according to a posterior of the Dirichlet distribution\cite{hsu2019measuring}, which divides clients into ten groups with different label distributions. Eight groups of clients will participate in the collaborative training process, and the rest will be held for test. % An example of the client setting is in Figure.\ref{fig-client-settings}.

% \begin{figure}[ht]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=\columnwidth]{images/exp/settings/client_settings.png}}
% \caption{Client settings} %  (b) shifts in the distributions of classes ; (c) shifts in the distributions of features. $\mathbf{p}$ and $\mathbf{q}$ are directions describing client-specific/-irrelevant knowledge. 
% \label{fig-client-settings}
% \end{center}
% \vskip -0.2in
% \end{figure}

\item \textbf{Feature-shift}: We experiment on the Digit-5 dataset to evaluate FedCS's performance on feature-shift data. The Digit-5 consists of digits from five domains (MNIST, MNIST-M, SVHN, USPS and Synth Digits). We assign instances of each domain to nine clients, where eight clients will train the global model and one for the test. In addition, we randomly draw instances from all domains to compose five mixed datasets for the test.
\end{itemize}

\subsection{Models and Hyperparameters}
We apply convolution neural networks (CNN) as fundamental models and integrate our proposed RA module into fully connected layers (FCs) to align their hidden layers (see Appendix for details of model architectures). By default, in each communication round, we sample ten clients to update the global model and evaluate the global model's performance on all clients. One epoch of fine-tuning steps will be applied for benchmark methods where the global model must be adapted to a client's local data before testing. The learning rate of a client's local training step is initialized as 0.005, and it will decay at the rate of 0.8 every 50 communication rounds. The RA module will be updated every five communication rounds by the sampled ten clients, and the learning rate is fixed at 0.001. (see Appendix for details of other hyperparameters).

% \begin{table}[t]
% \centering
% \caption{Hyperparamters for experiments}
% \label{table-hyperpara}
%\resizebox{.95\columnwidth}{!}{
% \begin{tabular}{l|c|c|c}
%     ~ & MNIST & CIFAR-10 & Digit-5\\
%     \hline
%     Rounds & 200 & 400 & 400 \\
%     Epoch/round & 5 & 30 & 10 \\
%     Batch Size & 10 & 32 & 10 \\
% \end{tabular}
% \end{table}




%\begin{figure}[t]
%\begin{minipage}[b]{1.0\linewidth}
% \centerline{\epsfig{figure=images/fedbn-cifar10.pdf}}
%\centerline{\includegraphics[width=2.0\columnwidth,]{images/fedbn-cifar10.png}}
%\caption{Weighted F1-scores within each client group (different colours). The horizontal axis denotes communication rounds, and the vertical axis denotes F1 Scores. } %  (b) shifts in the distributions of classes ; (c) shifts in the distributions of features. $\mathbf{p}$ and $\mathbf{q}$ are directions describing client-specific/-irrelevant knowledge. 
%\label{fig-grouped-f1-score-cifar10}
%\end{figure}

\begin{figure*}[ht]
%\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=2.0\columnwidth,]{images/fedbn-cifar10.png}}
\caption{Part of experiments on CIFAR-10. The horizontal axis denotes communication rounds, and the vertical axis denotes F1 Scores. We demonstrate the averaged weighted F1-scores within each client group and marked them with different colours. We can find the performance on different distributions (client groups) vary significantly through FedAvg+FT and FedBN. FedCS has the most robust performance even on unseen clients (group 8 and 9)} %  (b) shifts in the distributions of classes ; (c) shifts in the distributions of features. $\mathbf{p}$ and $\mathbf{q}$ are directions describing client-specific/-irrelevant knowledge. 
\label{fig-grouped-f1-score-cifar10}
\end{center}
%\vskip -0.2in
\end{figure*}

\subsection{Performance}
We first demonstrate averaged model performance on all clients, which shows that a global model learned with FedCS will achieve comparable performance to other personalized FL methods that require model adaptation. Then, we look inside the group-wised metrics to evaluate a model's performance on different distributions. The global model learned with FedCS is more robust to different distributions. It can be directly deployed on test clients without extra adaptation. Several FL strategies are compared as baselines: %1) FedAvg~\cite{mcmahan2017communication};
1) FedAvg+FT~\cite{cheng2021fine}; 2) FedAvg+BN; 3) FedBN~\cite{li2021fedbn}. %5) FedProx~\cite{li2018federated};
4) FedRep~\cite{collins2021exploiting}; 5) PerFL~\cite{pillutla2022federated}; 6) In addition, we demonstrate the performance of models those trained on each client locally (Local Only).

\subsection{Label-shift Settings}
\subsubsection{Overall Performance}
For label-shift settings, the weighted AUC score and the weighted F1 score are applied to evaluate model performance on data with unbalanced label distributions.
% \footnote{accuracy and other metrics are demonstrated in Appendix}.
Table.\ref{table-averaged-mnist} demonstrates models' performance on the MNIST dataset. We can find that a model with FedCS layers achieves the best performance under the label-shift setting. It outperforms those locally fine-tuned global models (FedAvg+FT) and models with client-specific parameters (FedBN). FedRep has the worst performance, which may result from the lack of training data and the unbalanced label distribution of each client.

\begin{table}[t]
\centering
\caption{The averaged performance on the MNIST dataset. The standard deviation of the metric between clients is reported in parentheses. w. is the abbreviation of 'weighted', and the $\uparrow$ denotes that the higher the metric is, the better performance a model achieved, and the best performance is highlighted.}
\label{table-averaged-mnist}
%\resizebox{.95\columnwidth}{!}{
\begin{tabular}{l|c|c}
    ~            & w. AUC ($10^{-2}$) $\uparrow$     & w. F1 ($10^{-2}$) $\uparrow$ \\
    \hline
    Local Only          & 85.18(4.62)    &47.80(10.12)\\
    % FedAvg              & 97.12(1.33)    &81.01(5.48)\\
    FedAvg+FT           & 96.97(2.54)    &80.81(10.14) \\
    FedAvg+BN           & 99.69(0.14)    &93.38(1.76) \\
    FedBN               & 99.32(0.75)    &83.85(18.82)\\
%    FedProx             & --(--)    &--.--(--.--)\\ 
    FedRep              & 75.72(15.56)   &38.53(20.52)\\
    PerFL               & 99.48(0.20)    &91.40(1.95)\\ 
%    FedBN+FT            & \bf{99.74}(0.13)    &93.64(1.59)\\
    \hline
    FedCS-FC1(ours)     & \bf{99.72(0.15)}    &\bf{93.72}(1.71)\\
    FedCS-FC2(ours)     & 99.71(0.16)    &93.43(1.78)\\
    FedCS-FC3(ours)     & 99.72(0.26)    &93.64(1.56)\\
\end{tabular}

\end{table}

Table.\ref{table-averaged-cifar10} demonstrates models' performance on the CIFAR-10 dataset. FedCS has the best performance under this setting. Other models are less effective than FedCS, and their performances vary significantly among clients (higher standard deviations). We will show that the gap results from the generalization error on test clients, and there is no such problem for the proposed FedCS.

\begin{table}[t]
\centering
\caption{The averaged performance on the CIFAR-10 dataset. The standard deviation of the metric between clients is reported in parentheses. w. is the abbreviation of 'weighted', and the $\uparrow$ denotes that the higher the metric is, the better performance a model achieved, and the best performance is highlighted.}
\label{table-averaged-cifar10}
%\resizebox{.95\columnwidth}{!}{
\begin{tabular}{l|c|c}
    ~            & w. AUC ($10^{-2}$)$\uparrow$     & w. F1 ($10^{-2}$)$\uparrow$ \\
    \hline
    Local Only          & 70.93(9.23)    &34.86(10.71)\\
    % FedAvg              & 88.03(3.61)    &54.04(8.61)\\
    FedAvg+FT           & 86.89(4.65)    &51.75(12.62) \\
    FedAvg+BN           & 91.57(4.30)    &57.87(14.95) \\
    FedBN               & 91.64(4.56)    &59.41(14.70)\\
    % FedProx             & 86.04(4.80)    &51.34(11.07)\\ 
    FedRep              & 70.70(9.80)    &33.01(13.88)\\
    PerFL               & 89.18(3.36)    &58.62(9.17)\\ 
%    FedBN+FT            & \bf{94.61}(2.10)    &\bf{71.61}(5.61)\\
    \hline
    FedCS-FC1(ours)     & \bf{93.72}(1.71)    &69.48(4.69)\\
    FedCS-FC2(ours)     & 93.33(2.33)    &69.06(5.97)\\
    FedCS-FC3(ours)     & 93.49(2.09)    &\bf{69.69(4.96)}\\
\end{tabular}

\end{table}


\begin{table}[t]
\centering
\caption{The averaged accuracy on the Digit-5 dataset. The standard deviation of the metric between clients is reported in parentheses. w. is the abbreviation of 'weighted', and the $\uparrow$ denotes that the higher the metric is, the better performance a model achieved, and the best performance is highlighted.}
\label{table-averaged-digit5}
%\resizebox{.95\columnwidth}{!}{
\begin{tabular}{l|c|c}
    ~            & w. AUC ($10^{-2}$)$\uparrow$     & w. F1 ($10^{-2}$)$\uparrow$ \\
    \hline
    Local Only          & 84.03(9.75)    &49.73(20.38)\\
    % FedAvg              & 98.16(1.43)    &85.69(6.38)\\
    FedAvg+FT           & 96.11(1.98)    &75.64(4.94) \\
    FedAvg+BN           & 97.82(3.11)    &83.40(12.96) \\
    FedBN               & 95.71(3.79)    &74.07(10.90)\\
    % FedProx             & --(--)    &--.--(--.--)\\ 
    FedRep              & 82.94(11.54)   &50.14(20.88)\\
    PerFL               & 96.10(2.47)    &74.63(6.71)\\ 
%    FedBN+FT            & \bf{94.61}(2.10)    &\bf{71.61}(5.61)\\
    \hline
    FedCS-FC1(ours)     & \bf{98.74}(0.95)    &\bf{87.89}(4.76)\\
    FedCS-FC2(ours)     & 98.60(1.09)    &87.66(5.15)\\
    FedCS-FC3(ours)     & 98.57(1.09)    &87.66(5.19)\\
\end{tabular}

\end{table}



% \begin{table}[t]
% \begin{center}
% \caption{Table caption} \label{tab:cap}
% \begin{tabular}{|c|c|c|}
%   \hline
  % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
%   Column One & Column Two & Column Three
%   \\
%   \hline
%   Cell 1 & Cell 2 & Cell 3 \\
%   Cell 4 & Cell 5 & Cell 6 \\
%   \hline
% \end{tabular}
% \end{center}
% \end{table}


% \begin{figure*}[ht]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=2.0\columnwidth,height=10cm]{images/exp/classification/digit5_acc/Digit-5.pdf}}
% \caption{Accuracy within each client group. We demonstrate the mean accuracy of clients from the same domain. Dashed lines denote the mean of accuracy on test clients. Shades denote the standard deviation of accuracy among clients.} %  (b) shifts in the distributions of classes ; (c) shifts in the distributions of features. $\mathbf{p}$ and $\mathbf{q}$ are directions describing client-specific/-irrelevant knowledge. 
% \label{fig-grouped-acc-digit-5}
% \end{center}
% \vskip -0.2in
% \end{figure*}


\subsubsection{Group-wised Performance}
Fig.\ref{fig-grouped-f1-score-cifar10} demonstrates averaged weighted F1-scores within each client group\footnote{Full version of results are shown in Appendix.}. We can find that the global model with FedCR is more robust among different clients, even if they are from test groups (groups 8-9). Fine-tuned models (FedAvg+FT) and models with personalized parameters (FedBN) have significant performance gaps when deployed on training clients (group 0-7) and test clients. They achieve higher F1 scores in training groups but could be less effective in test groups.



\subsection{Feature-shift Settings}
In this section, we demonstrate evaluations of feature-shifted data. According to Table.\ref{table-averaged-digit5}, we show that FedCS achieves the highest weighted AUC and weighted-F1 score. The averaged accuracy within each data domain is shown in the Appendix. %Figure.\ref{fig-grouped-acc-digit-5}.
It also validates our claims that FedCS performs more robustly on all domains while other methods degenerate significantly on test clients. %(dash lines). %\footnote{Due to limited space, more comparisons and high-resolution results are given in the appendix.}

